Text2Shape: Generating Shapes from Natural Language by Learning Joint Embeddings

We present a method for generating colored 3D shapes from natural language. To this end, we first learn joint embeddings of freeform text descriptions and colored 3D shapes. Our model combines and extends learning by association and metric learning approaches to learn implicit cross-modal connections, and produces a joint representation that captures the many-to-many relations between language and physical properties of 3D shapes such as color and shape. To evaluate our approach, we collect a large dataset of natural language descriptions for physical 3D objects in the ShapeNet dataset. With this learned joint embedding we demonstrate text-to-shape retrieval that outperforms baseline approaches. Using our embeddings with a novel conditional Wasserstein GAN framework, we generate colored 3D shapes from text. Our method is the first to connect natural language text with realistic 3D objects exhibiting rich variations in color, texture, and shape detail. See video at https://youtu.be/zraPvRdl13Q

==> fig/primitives-cross-modal-retrieval.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{fig/primitives-text-shape-retrieval_3.pdf}
    \caption{\textbf{Text-to-shape retrieval.} We show the five nearest neighbors to the text using our learned embedding. The shapes are correctly retrieved and match the query text.}
    \label{fig:primitives-cross-modal-retrieval}
\end{figure}

==> fig/primitives-shape-shape-retrieval.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{fig/primitives-shape-shape-retrieval.pdf}
    \caption{\textbf{Shape-to-shape retrieval.} Using our method for the primitives dataset, the nearest neighbor shapes usually match the query exactly. Each retrieved model is slightly different from the query but still comes from the same configuration}
    \label{fig:primitives-shape-shape-retrieval}
\end{figure}

==> fig/primitives-text-text-retrieval.tex <==
\begin{figure}
    \includegraphics[width=\linewidth]{fig/primitives-text-text-retrieval.pdf}
    \caption{\textbf{Text-to-text retrieval.} The retrieved descriptions come from the same configuration as the query when using our method. %(except for one retrieved description).
    %\todo{Cut down to only nearest neighbor?, move to supplemental}
    }
    \label{fig:primitives-text-text-retrieval}
\end{figure}

==> fig/shape_editing_old.tex <==
\begin{figure}
    \vspace{-1.5em}
	\captionsetup[subfigure]{justification=centering,labelformat=empty}
	\centering
	\begin{subfigure}[t]{0.18\linewidth}
		\includegraphics[width=\linewidth]{fig/custom_desc/tables/0050_voxel_tensor_output.png}
		\caption{\scriptsize{\emph{White coffee table}}}
	\end{subfigure}
	\begin{subfigure}[t]{0.18\linewidth}
		\includegraphics[width=\linewidth]{fig/custom_desc/tables/0056_voxel_tensor_output.png}
		\caption{\scriptsize{\emph{Wooden coffee table}}}
	\end{subfigure}
	\begin{subfigure}[t]{0.18\linewidth}
        \includegraphics[width=\linewidth]{fig/custom_desc/tables/0009_voxel_tensor_output.png}
        \caption{\scriptsize{\emph{Rectangular glass coffee table}}}
	\end{subfigure}
	\begin{subfigure}[t]{0.18\linewidth}
		\includegraphics[width=\linewidth]{fig/custom_desc/tables/0171_voxel_tensor_output.png}
		\caption{\scriptsize{\emph{Glass round coffee table}}}
	\end{subfigure}
	\begin{subfigure}[t]{0.18\linewidth}
		\includegraphics[width=\linewidth]{fig/custom_desc/tables/0191_voxel_tensor_output.png}
		\caption{\scriptsize{\emph{Red round coffee table}}}
	\end{subfigure}
	
	% Chairs
% 	\begin{subfigure}[t]{0.125\linewidth}
% 		\includegraphics[width=\linewidth]{fig/custom_desc/chairs/0085_voxel_tensor_output.png}
% 		\caption{\scriptsize{\emph{Gray chair}}}
% 	\end{subfigure}
	\begin{subfigure}[t]{0.18\linewidth}
		\includegraphics[width=\linewidth]{fig/custom_desc/chairs/0100_voxel_tensor_output.png}
		\caption{\scriptsize{\emph{Red chair}}}
	\end{subfigure}
	\begin{subfigure}[t]{0.18\linewidth}
		\includegraphics[width=\linewidth]{fig/custom_desc/chairs/0007_voxel_tensor_output.png}
		\caption{\scriptsize{\emph{Dining chair}}}
	\end{subfigure}
% 	\begin{subfigure}[t]{0.125\linewidth}
% 		\includegraphics[width=\linewidth]{fig/custom_desc/chairs/0017_voxel_tensor_output.png}
% 		\caption{\scriptsize{\emph{Gray dining chair}}}
% 	\end{subfigure}
	\begin{subfigure}[t]{0.18\linewidth}
		\includegraphics[width=\linewidth]{fig/custom_desc/chairs/0036_voxel_tensor_output.png}
		\caption{\scriptsize{\emph{Gray dining chair}}}
	\end{subfigure}
	\begin{subfigure}[t]{0.18\linewidth}
		\includegraphics[width=\linewidth]{fig/custom_desc/chairs/0023_voxel_tensor_output.png}
		\caption{\scriptsize{\emph{Silver leather chair}}}
	\end{subfigure}
% 	\begin{subfigure}[t]{0.125\linewidth}
% 		\includegraphics[width=\linewidth]{fig/custom_desc/chairs/0043_voxel_tensor_output.png}
% 		\caption{\scriptsize{\emph{Silver leather chair}}}
% 	\end{subfigure}
% 	\begin{subfigure}[t]{0.125\linewidth}
% 		\includegraphics[width=\linewidth]{fig/custom_desc/chairs/0044_voxel_tensor_output.png}
% 		\caption{\scriptsize{\emph{Silver leather chair}}}
% 	\end{subfigure}
	\begin{subfigure}[t]{0.17\linewidth}
		\includegraphics[width=\linewidth]{fig/custom_desc/chairs/0072_voxel_tensor_output.png}
		\caption{\scriptsize{\emph{Gray leather chair}}}
	\end{subfigure}
% 	\begin{subfigure}[t]{0.125\linewidth}
% 		\includegraphics[width=\linewidth]{fig/custom_desc/chairs/0079_voxel_tensor_output.png}
% 		\caption{\scriptsize{\emph{Gray leather chair}}}
% 	\end{subfigure}
    \vspace{-1em}
    \caption{As different attributes are described in the descriptions, the generated shapes reflect those changes.}
    \label{fig:shape-editing}
    \vspace{-1.5em}
\end{figure}


==> fig/text-text-retrieval-comparison.tex <==
\begin{figure}
    \includegraphics[width=\linewidth]{fig/text-text-retrieval-comparison.pdf}
    \caption{\textbf{Text-to-text retrieval.} We compare our method with the LBA (TST) and DS-SJE baselines~\cite{reed2016learning}. The LBA (TST) method works fairly well for this task, but struggles with other retrieval tasks. Our method works well for all retrieval tasks.%(except for one retrieved description).
    %\todo{Cut down to only nearest neighbor?, move to supplemental}
    }
    \label{fig:text-text-retrieval-comparison}
\end{figure}

==> fig/text2shape_results_backup.tex <==
\begin{figure}
    \centering\footnotesize
    \aboverulesep=.5mm \belowrulesep=.5mm
    \vspace{-1em}
    \begin{tabular}{cccc}
    GAN-CLS~\cite{reed2016generative} & Ours CGAN & Ours CWGAN & GT
    \\\toprule

    \multicolumn{4}{c}{Dark brown wooden dining chair with red padded}\\
    \multicolumn{4}{c}{seat and round red pad back.\vspace{-1em}}\\
    \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/reed/0007_voxel_tensor_output.png} &
    \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/cgan/0007_voxel_tensor_output.png} &
    \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/iwgan/0007_voxel_tensor_output.png} &
    \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/gt/0007_voxel_tensor_fake_match.png}
    \vspace{-1em}
    % \\\midrule
    % \multicolumn{4}{c}{This table is gray and is made out of metal. It has four legs}\\
    % \multicolumn{4}{c}{sticking out of the bottom but it has four circular feet which are colored peach.}\\
    % \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/reed/0020_voxel_tensor_output.png} &
    % \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/cgan/0020_voxel_tensor_output.png} &
    % \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/iwgan/0020_voxel_tensor_output.png} &
    % \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/gt/0020_voxel_tensor_fake_match.png}

    \\\midrule
    \multicolumn{4}{c}{Circular table, I would expect to see}\\
    \multicolumn{4}{c}{couches surrounding this type of table.\vspace{-1em}}\\
    \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/reed/0061_voxel_tensor_output.png} &
    \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/cgan/0061_voxel_tensor_output.png} &
    \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/iwgan/0061_voxel_tensor_output.png} &
    \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/gt/0061_voxel_tensor_fake_match.png}
    \vspace{-0.5em}

    \\\midrule
    \multicolumn{4}{c}{Waiting room chair leather}\\
    %\multicolumn{4}{c}{legs and armrests are curved wood.\vspace{-1em}}\\
    \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/reed/0003_voxel_tensor_output.png} &
    \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/cgan/0003_voxel_tensor_output.png} &
    \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/iwgan/0003_voxel_tensor_output.png} &
    \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/gt/0003_voxel_tensor_fake_match.png}
    \vspace{-0.5em}

    % \\\midrule
    % \multicolumn{4}{c}{This is a brown chair that would be a diner chair. Its back}\\
    % \multicolumn{4}{c}{is made of horizontal slats. It is brown and made of wood.\vspace{-1em}}\\
    % \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/reed/0056_voxel_tensor_output.png} &
    % \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/cgan/0056_voxel_tensor_output.png} &
    % \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/iwgan/0056_voxel_tensor_output.png} &
    % \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/gt/0056_voxel_tensor_fake_match.png}
    % \vspace{-0.5em}

    \\\midrule
    \multicolumn{4}{c}{A multi-layered end table made of cherry wood. There is}\\
    \multicolumn{4}{c}{a rectangular surface with curved ends, and a square storage}\\
    \multicolumn{4}{c}{surface underneath that is slightly smaller.\vspace{-1em}}\\
    \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/reed/0094_voxel_tensor_output.png} &
    \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/cgan/0094_voxel_tensor_output.png} &
    \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/iwgan/0094_voxel_tensor_output.png} &
    \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/gt/0094_voxel_tensor_fake_match.png}
    \vspace{-0.5em}

    \\\midrule
    \multicolumn{4}{c}{Brown colored dining table. It has four legs made of wood.\vspace{-0.5em}}\\
    \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/reed/0045_voxel_tensor_output.png} &
    \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/cgan/0045_voxel_tensor_output.png} &
    \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/iwgan/0045_voxel_tensor_output.png} &
    \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/gt/0045_voxel_tensor_fake_match.png}
    \vspace{-1em}

    % \\\midrule
    % \multicolumn{4}{c}{It's a table with bar legs and a flat top. It's white in color}\\
    % \multicolumn{4}{c}{and has a brace on the back for extra support, and has leg room underneath.}\\
    % \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/reed/0100_voxel_tensor_output.png} &
    % \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/cgan/0100_voxel_tensor_output.png} &
    % \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/iwgan/0100_voxel_tensor_output.png} &
    % \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/gt/0100_voxel_tensor_fake_match.png}

    \end{tabular}
    \caption{\textbf{Example text-to-shape generations}. Our CWGAN approach is correctly conditioned by the input text, generating shapes that match the described attributes.The baseline approach does not generate plausible shapes.}
    \vspace{-1.5em}
    \label{fig:text2shape_results}
\end{figure}


==> fig/text2shape_results_side_by_side.tex <==
\begin{figure}
    \captionsetup[subfigure]{justification=centering,labelformat=empty}
    \centering\footnotesize
    % \vspace{-1em}
    \begin{subfigure}[t]{0.4\linewidth}
        \centering
        \aboverulesep=.5mm \belowrulesep=.5mm
        \begin{tabular}{cccc}
        GAN-CLS~\cite{reed2016generative} & Ours CGAN & Ours CWGAN & GT
        \\\toprule
    
        \multicolumn{4}{c}{Dark brown wooden dining}\\
        \multicolumn{4}{c}{chair with red padded}\\
        \multicolumn{4}{c}{seat and round red pad back.\vspace{-1em}}\\
        \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/reed/0007_voxel_tensor_output.png} &
        \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/cgan/0007_voxel_tensor_output.png} &
        \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/iwgan/0007_voxel_tensor_output.png} &
        \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/gt/0007_voxel_tensor_fake_match.png}
        \vspace{-1em}
        % \\\midrule
        % \multicolumn{4}{c}{This table is gray and is made out of metal. It has four legs}\\
        % \multicolumn{4}{c}{sticking out of the bottom but it has four circular feet which are colored peach.}\\
        % \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/reed/0020_voxel_tensor_output.png} &
        % \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/cgan/0020_voxel_tensor_output.png} &
        % \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/iwgan/0020_voxel_tensor_output.png} &
        % \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/gt/0020_voxel_tensor_fake_match.png}
    
        \\\midrule
        \multicolumn{4}{c}{Circular table, I would expect to see}\\
        \multicolumn{4}{c}{would expect to see}\\
        \multicolumn{4}{c}{couches surrounding this}\\
        \multicolumn{4}{c}{type of table.\vspace{-1em}}\\
        \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/reed/0061_voxel_tensor_output.png} &
        \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/cgan/0061_voxel_tensor_output.png} &
        \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/iwgan/0061_voxel_tensor_output.png} &
        \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/gt/0061_voxel_tensor_fake_match.png}
        \vspace{-0.5em}
    
        \\\midrule
        \multicolumn{4}{c}{Waiting room chair leather}\\
        %\multicolumn{4}{c}{legs and armrests are curved wood.\vspace{-1em}}\\
        \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/reed/0003_voxel_tensor_output.png} &
        \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/cgan/0003_voxel_tensor_output.png} &
        \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/iwgan/0003_voxel_tensor_output.png} &
        \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/gt/0003_voxel_tensor_fake_match.png}
        \end{tabular}
        \vspace{-0.5em}
    \end{subfigure}
    \begin{subfigure}[t]{0.4\linewidth}
        \centering
        \begin{tabular}{cccc}
        GAN-CLS~\cite{reed2016generative} & Ours CGAN & Ours CWGAN & GT
        \\\toprule
        % \\\midrule
        % \multicolumn{4}{c}{This is a brown chair that would be a diner chair. Its back}\\
        % \multicolumn{4}{c}{is made of horizontal slats. It is brown and made of wood.\vspace{-1em}}\\
        % \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/reed/0056_voxel_tensor_output.png} &
        % \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/cgan/0056_voxel_tensor_output.png} &
        % \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/iwgan/0056_voxel_tensor_output.png} &
        % \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/gt/0056_voxel_tensor_fake_match.png}
        % \vspace{-0.5em}
    
        % \\\midrule
        \multicolumn{4}{c}{A multi-layered end table}\\
        \multicolumn{4}{c}{ made of cherry wood.}\\
        \multicolumn{4}{c}{There is a rectangular}\\
        \multicolumn{4}{c}{surface with curved ends,}\\
        \multicolumn{4}{c}{and a square storage}\\
        \multicolumn{4}{c}{surface underneath that}\\
        \multicolumn{4}{c}{is slightly smaller.\vspace{-1em}}\\
        \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/reed/0094_voxel_tensor_output.png} &
        \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/cgan/0094_voxel_tensor_output.png} &
        \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/iwgan/0094_voxel_tensor_output.png} &
        \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/gt/0094_voxel_tensor_fake_match.png}
        \vspace{-0.5em}
    
        \\\midrule
        \multicolumn{4}{c}{Brown colored dining}\\
        \multicolumn{4}{c}{table. It has four legs}\\
        \multicolumn{4}{c}{made of wood.\vspace{-0.5em}}\\
        \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/reed/0045_voxel_tensor_output.png} &
        \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/cgan/0045_voxel_tensor_output.png} &
        \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/iwgan/0045_voxel_tensor_output.png} &
        \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/gt/0045_voxel_tensor_fake_match.png}
        \vspace{-1em}
    
        % \\\midrule
        % \multicolumn{4}{c}{It's a table with bar legs and a flat top. It's white in color}\\
        % \multicolumn{4}{c}{and has a brace on the back for extra support, and has leg room underneath.}\\
        % \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/reed/0100_voxel_tensor_output.png} &
        % \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/cgan/0100_voxel_tensor_output.png} &
        % \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/iwgan/0100_voxel_tensor_output.png} &
        % \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/gt/0100_voxel_tensor_fake_match.png}
    
        \end{tabular}
    \end{subfigure}
    \caption{\textbf{Example text-to-shape generations}. Our CWGAN approach is correctly conditioned by the input text, generating shapes that match the described attributes.The baseline approach does not generate plausible shapes.}
    \vspace{-1.5em}
    \label{fig:text2shape_results}
\end{figure}


==> fig/text2shape_results_wide.tex <==
\begin{figure}
    \centering\footnotesize
    \aboverulesep=.5mm \belowrulesep=.5mm
    \vspace{-1em}
    % \begin{tabular}{\textwidth}{@{\extracolsep{\textwidth minus\textwidth}}*4{c}@{}}
    \begin{tabularx}{\textwidth}{*{4}{>{\centering\arraybackslash}X}}
    GAN-CLS~\cite{reed2016generative} & Ours CGAN & Ours CWGAN & GT\\
    \toprule

    \multicolumn{4}{c}{Dark brown wooden dining chair with red padded seat and round red pad back.\vspace{-1em}}\\
    \adjincludegraphics[width=0.5\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/reed/0007_voxel_tensor_output.png} &
    \adjincludegraphics[width=0.5\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/cgan/0007_voxel_tensor_output.png} &
    \adjincludegraphics[width=0.5\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/iwgan/0007_voxel_tensor_output.png} &
    \adjincludegraphics[width=0.5\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/gt/0007_voxel_tensor_fake_match.png}
    \vspace{-1em}
    % \\\midrule
    % \multicolumn{4}{c}{This table is gray and is made out of metal. It has four legs}\\
    % \multicolumn{4}{c}{sticking out of the bottom but it has four circular feet which are colored peach.}\\
    % \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/reed/0020_voxel_tensor_output.png} &
    % \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/cgan/0020_voxel_tensor_output.png} &
    % \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/iwgan/0020_voxel_tensor_output.png} &
    % \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/gt/0020_voxel_tensor_fake_match.png}

    \\\midrule
    \multicolumn{4}{c}{Circular table, I would expect to see couches surrounding this type of table.\vspace{-1em}}\\
    \adjincludegraphics[width=0.5\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/reed/0061_voxel_tensor_output.png} &
    \adjincludegraphics[width=0.5\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/cgan/0061_voxel_tensor_output.png} &
    \adjincludegraphics[width=0.5\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/iwgan/0061_voxel_tensor_output.png} &
    \adjincludegraphics[width=0.5\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/gt/0061_voxel_tensor_fake_match.png}
    \vspace{-0.5em}

    \\\midrule
    \multicolumn{4}{c}{Waiting room chair leather}\\
    %\multicolumn{4}{c}{legs and armrests are curved wood.\vspace{-1em}}\\
    \adjincludegraphics[width=0.5\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/reed/0003_voxel_tensor_output.png} &
    \adjincludegraphics[width=0.5\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/cgan/0003_voxel_tensor_output.png} &
    \adjincludegraphics[width=0.5\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/iwgan/0003_voxel_tensor_output.png} &
    \adjincludegraphics[width=0.5\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/gt/0003_voxel_tensor_fake_match.png}
    \vspace{-0.5em}

    % \\\midrule
    % \multicolumn{4}{c}{This is a brown chair that would be a diner chair. Its back}\\
    % \multicolumn{4}{c}{is made of horizontal slats. It is brown and made of wood.\vspace{-1em}}\\
    % \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/reed/0056_voxel_tensor_output.png} &
    % \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/cgan/0056_voxel_tensor_output.png} &
    % \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/iwgan/0056_voxel_tensor_output.png} &
    % \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/gt/0056_voxel_tensor_fake_match.png}
    % \vspace{-0.5em}

    \\\midrule
    \multicolumn{4}{c}{A multi-layered end table made of cherry wood. There is a rectangular surface with}\\
    \multicolumn{4}{c}{curved ends, and a square storage surface underneath that is slightly smaller.\vspace{-1em}}\\
    \adjincludegraphics[width=0.5\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/reed/0094_voxel_tensor_output.png} &
    \adjincludegraphics[width=0.5\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/cgan/0094_voxel_tensor_output.png} &
    \adjincludegraphics[width=0.5\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/iwgan/0094_voxel_tensor_output.png} &
    \adjincludegraphics[width=0.5\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/gt/0094_voxel_tensor_fake_match.png}
    \vspace{-0.5em}

    \\\midrule
    \multicolumn{4}{c}{Brown colored dining table. It has four legs made of wood.\vspace{-0.5em}}\\
    \adjincludegraphics[width=0.5\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/reed/0045_voxel_tensor_output.png} &
    \adjincludegraphics[width=0.5\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/cgan/0045_voxel_tensor_output.png} &
    \adjincludegraphics[width=0.5\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/iwgan/0045_voxel_tensor_output.png} &
    \adjincludegraphics[width=0.5\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/gt/0045_voxel_tensor_fake_match.png}
    \vspace{-1em}

    % \\\midrule
    % \multicolumn{4}{c}{It's a table with bar legs and a flat top. It's white in color}\\
    % \multicolumn{4}{c}{and has a brace on the back for extra support, and has leg room underneath.}\\
    % \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/reed/0100_voxel_tensor_output.png} &
    % \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/cgan/0100_voxel_tensor_output.png} &
    % \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/iwgan/0100_voxel_tensor_output.png} &
    % \adjincludegraphics[width=0.17\linewidth,trim={{.05\width} {.05\height} {.05\width} {.05\height}},clip]{fig/results/gt/0100_voxel_tensor_fake_match.png}

    \end{tabularx}
    \caption{\textbf{Text-to-shape generation results}. Our CWGAN approach is correctly conditioned by the input text, generating shapes that match the described attributes. The baseline approach does not generate plausible shapes.}
    \vspace{-1.5em}
    \label{fig:text2shape_results}
\end{figure}


==> tab/primitives-text-text-retrieval.tex <==
\begin{table*}
    \begin{center}
    \caption{\textbf{Text-to-text retrieval.} The retrieved descriptions come from the same configuration as the query when using our method. %(except for one retrieved description).
    %\todo{Cut down to only nearest neighbor?, move to supplemental}
    }
    \label{fig:primitives-text-text-retrieval}
    % \label{tab:retrieval-same-modal}
    \small
        \begin{tabular}{|p{2cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|}
        \toprule
        \textbf{Query} & \multicolumn{5}{c|}{\textbf{Nearest Neighbors}} \\
        % \cmidrule(l){1} \cmidrule(l){2-3}
        \midrule
        a large jade wide cube & the large rectangular shape is wide jade & the large rectangular shape is broad jade & a large broad jade box & a large wide jade box & a large wide green box\\
        \midrule
        a large squat bleached wide conical shape & a large short bleached wide conical shape & a large low bleached broad conical shape & a large short bleached broad conical shape & a large squat bleached broad conical shape & a large low bleached wide conical shape\\
        \midrule
        the narrow blue-green sphere is tall & the thin spherical shape is high cerulean & the thin spherical shape is high blue-green & the thin spherical shape is tall cerulean & the narrow spherical shape is high cerulean & the thin round shape is high cerulean\\
        \bottomrule
        \end{tabular}
    \end{center}
\end{table*}

==> tab/retrieval-text-shape.tex <==
\begin{table*}
\begin{center}
\caption{\textbf{Text-to-shape retrieval results on the primitives dataset.} Our approach significantly outperforms baselines from prior work.}
\label{tab:text-shape-retrieval}
\small
\begin{tabular}{lccc}
\toprule
Method & RR@1 & RR@5 & NDCG@5 \\
\midrule
Random & 0.24 & 0.76 & 0.27 \\
%Word2vec & foo & bar & foo & N/A & N/A & N/A & N/A & N/A & N/A \\
DS-SJE~\cite{reed2016learning} & 81.77 & 90.70 & 81.29 \\
LBA (TST)~\cite{haeusser2017learning} & 5.06 & 15.29 & 5.92 \\
\midrule
ML & 25.93 & 57.24 & 25.00 \\
LBA (MM) & 91.13 & 98.27 & 91.90 \\
LBA+ML (TST) & 94.24 & 97.55 & 95.20 \\
LBA+ML (MM) & \textbf{95.07} & \textbf{99.08} & \textbf{95.51} \\
\bottomrule
\end{tabular}
\end{center}
\end{table*}


==> tab/retrieval.tex <==
\begin{table*}
\begin{center}
\caption{\textbf{Retrieval results on the primitives dataset.} Our approach significantly outperforms baselines from prior work.}
\label{tab:retrieval}
\small
\begin{tabular}{lccccccccc}
\toprule
 & \multicolumn{3}{c}{Text-to-text retrieval} & \multicolumn{3}{c}{Shape-to-shape retrieval} & \multicolumn{3}{c}{Text-to-shape retrieval}\\
\cmidrule(l){2-4} \cmidrule(l){5-7} \cmidrule(l){8-10}   
Method & RR@1 & RR@5 & NDCG@5 & RR@1 & RR@5 & NDCG@5 & RR@1 & RR@5 & NDCG@5 \\
\midrule
Random & 6.31 & 17.94 & 5.27 & 1.33 & 1.6 & 1.35 & 0.24 & 0.76 & 0.27 \\
%Word2vec & foo & bar & foo & N/A & N/A & N/A & N/A & N/A & N/A \\
DS-SJE~\cite{reed2016learning} & 35.41 & 43.38 & 35.05 & 37.87 & 46.00 & 35.48 & 81.77 & 90.70 & 81.29 \\
LBA (TST)~\cite{haeusser2017learning} & 23.16 & 24.18 & 23.21 & 13.47 & 29.07 & 12.06 & 5.06 & 15.29 & 5.92 \\
\midrule
ML & 24.01 & 28.31 & 23.73 & 30.93 & 64.27 & 29.60 & 25.93 & 57.24 & 25.00 \\
LBA (MM) & 61.84 & 62.71 & 62.03 & 20.80 & 28.00 & 18.94 & 91.13 & 98.27 & 91.90 \\
LBA+ML (TST) & \textbf{100} & \textbf{100} & \textbf{100} & \textbf{96.53} & 98.80 & 95.30 & 94.24 & 97.55 & 95.20 \\
LBA+ML (MM) & \textbf{100} & \textbf{100} & \textbf{100} & 96.13 & \textbf{99.20} & \textbf{95.59} & \textbf{95.07} & \textbf{99.08} & \textbf{95.51} \\
\bottomrule
\end{tabular}
\end{center}
\end{table*}


==> tab/shapenet-text-text-retrieval-comparison.tex <==
\begin{table*}
    \begin{center}
    \caption{\textbf{Text-to-text retrieval.} We compare our method with the LBA (TST) and DS-SJE baselines~\cite{reed2016learning}. The LBA (TST) method works fairly well for this task, but struggles with other retrieval tasks. Our method works well for all retrieval tasks.%(except for one retrieved description).
    %\todo{Cut down to only nearest neighbor?, move to supplemental}
    }
    \label{tab:text-text-retrieval-comparison}
    % \label{tab:retrieval-same-modal}
    \small
        \begin{tabular}{|p{1.5cm}|p{5cm}|p{5cm}|}
        \toprule
        \multicolumn{3}{|c|}{\textbf{Query}: Grey, circular table with a circular base with a rod supporting both} \\
        \midrule
        \textbf{Method} & \multicolumn{2}{c|}{\textbf{Nearest Neighbors}} \\
        % \cmidrule(l){1} \cmidrule(l){2-3}
        \midrule
        \textbf{LBA (TST)} & a silver table with circular glass top and square legs & This is a glass and metal coffee table. The table surface is glass while the legs is metal.\\
        \midrule
        \textbf{DS-SJE} & This is a short brown elongated Round Table. This table would be used as a coffee table with a small table in the middle of a room. & A white folding table that can be used a rectangular dining table or a round dining table.\\
        \midrule
        \textbf{Ours} & a round table, apparently made of plastic, light gray & A grey colored steel round table with two round surface and with four legs.\\
        \bottomrule
        \toprule
        \multicolumn{3}{|c|}{\textbf{Query}: Brown, rectangle, wood. It’s a chair that looks like it rocks and it is} \\
        \multicolumn{3}{|c|}{a light brown color.}\\
        \midrule
        \textbf{Method} & \multicolumn{2}{c|}{\textbf{Nearest Neighbors}} \\
        % \cmidrule(l){1} \cmidrule(l){2-3}
        \midrule
        \textbf{LBA (TST)} & Medium brown color,woodenchair. Square seat, slatted wooden back, with curved wooden top. Four spindle type wooden legs. & Brown, wood chair with a straight back made of 5 dowels. Resembles a dining room chair.\\
        \midrule
        \textbf{DS-SJE} & White chair made of plastic that aligns the seat and back of the chair. The wooden frame of the chair supports the chair with its 4 small wooden legs. & Brown colored wooden chair with flat seat and back rest and armless chair. Four short legs and back side of the chair being ash grey colored.\\
        \midrule
        \textbf{Ours} & White chair made of plastic that aligns the seat and back of the chair. The wooden frame of the chair supports the chair with its 4 small wooden legs. & Teakwood, stain brown and stain yellow color, square and semi rectangle shape.\\
        \bottomrule
        \end{tabular}
    \end{center}
\end{table*}

==> tab/shapenet-text-text-retrieval.tex <==
\begin{table*}
    \begin{center}
    \caption{\textbf{Text-to-text retrieval.} The retrieved descriptions are semantically similar to the query despite originating from different shape instances. %(except for one retrieved description).
    %\todo{Cut down to only nearest neighbor?, move to supplemental}
    }
    \label{tab:text-text-retrieval}
    \small
        \begin{tabular}{|p{3cm}|p{4cm}|p{4cm}|}
        \toprule
        \textbf{Query} & \multicolumn{2}{c|}{\textbf{Nearest Neighbors}} \\
        \midrule
        % \cmidrule(l){1} \cmidrule(l){2-3}
        \midrule
        \textbf{an brown oval table with three section base} & The table is a sofa table with an oval top. The legs are rounded and the table is multi-colored wood. & Circulartable of beige colourwith 3 stand where the first two stands are circular and the bottonpart is rectangular and it is supported by a wooden broad c piece.\\
        \midrule
        \textbf{a red plastic seating unit in one piece, sitting on a metal frame for feet.} & A red metal chair with a red leg rest. The frame is made of one piece of metal that is bent for the shape. & A circular red chair with a small round base. The red chair has minimal padding and the inner seat base is black in colour.\\
        \midrule
        \textbf{a drawer, wooden color, used to keep things like books, clothes, it has three drawer} & A box with long hightdesk type table of teak color with three drawers and a tilted top & The table is made up of wood. It has one drawers. It is four legged\\
        \midrule
        \textbf{Light blue top glass coffee table with brown metallic stand.} & The modern design coffee table features wooden legs and a glass top and glass under shelf. The square wooden legs are black in color. & it is grey in color, rectangle in shape with modern manufactured allowing for versatile, striking designed with metal joints and top of the table is covered with glass and appearance looks like glass coffee table\\
        \bottomrule
        \end{tabular}
    \end{center}
\end{table*}
